Are we certain it's anomalous?

The progress in modelling time series and, more generally, sequences of structured data has recently revamped research in anomaly detection. The task stands for identifying abnormal behaviors in financial series, IT systems, aerospace measurements, and the medical domain, where anomaly detection may aid in isolating cases of depression and attend the elderly. Anomaly detection in time series is a complex task since anomalies are rare due to highly non-linear temporal correlations and since the definition of anomalous is sometimes subjective. Here we propose the novel use of Hyperbolic uncertainty for Anomaly Detection (HypAD). HypAD learns self-supervisedly to reconstruct the input signal. We adopt best practices from the state-of-the-art to encode the sequence by an LSTM, jointly learned with a decoder to reconstruct the signal, with the aid of GAN critics. Uncertainty is estimated end-to-end by means of a hyperbolic neural network. By using uncertainty, HypAD may assess whether it is certain about the input signal but it fails to reconstruct it because this is anomalous; or whether the reconstruction error does not necessarily imply anomaly, as the model is uncertain, e.g. a complex but regular input signal. The novel key idea is that a detectable anomaly is one where the model is certain but it predicts wrongly. HypAD outperforms the current state-of-the-art for univariate anomaly detection on established benchmarks based on data from NASA, Yahoo, Numenta, Amazon, and Twitter. It also yields state-of-the-art performance on a multivariate dataset of anomaly activities in elderly home residences, and it outperforms the baseline on SWaT. Overall, HypAD yields the lowest false alarms at the best performance rate, thanks to successfully identifying detectable anomalies.

==> fig/ablation.tex <==
\begin{figure}[] 
\begin{center}
	\includegraphics[width=0.5\textwidth]{fig/images/ablation2.pdf}
\end{center}
\caption{\BM{Qualitative Ablation on SWaT: The blue color represents the predicted anomaly scores, which we mark as red when it is above the anomaly detection threshold. That is, the red points denotes the predicted anomalies. The green points represents the ground-truth, where a value of 1 means anomaly and 0 means non-anomaly.}} 
\label{fig:ablation}
\end{figure}


==> sec/Backup/abs_bk_2022-02-09.tex <==
\begin{abstract}
The progress in modelling time series and, more generally, sequences of structured-data has recently revamped research in anomaly detection. The task stands for identifying abnormal behaviours in financial series, IT systems, aerospace measurements, and the medical domain, where anomaly detection may aid in isolating cases of depression and attend the elderly. Anomaly detection in time series is a complex task since anomalies are rare due to highly non-linear temporal correlations and since the definition of anomalous is sometimes subjective.

Here we propose the novel use of Hyperbolic uncertainty for Anomaly Detection (HypAD). HypAD learns self-supervisedly to reconstruct the input signal. 
We adopt best practices from the state-of-the-art to encode the sequence by an LSTM, jointly learnt with a decoder to reconstruct the signal, with the aid of GAN discriminators. The proposed hyperbolic uncertainty is integrated end-to-end and it allows HypAD to minimise the reconstruction loss, either by matching the signal exactly --resulting in zero loss-- or by reconstructing it with some error, but making the estimate less certain.
In fact, in the proposed hyperbolic formulation, the more certain is the model, the exponentially-larger is the penalisation for reconstruction errors.

Thanks to this principled formulation of uncertainty, HypAD outperforms the current state-of-the-art on established anomaly benchmarks based on data from NASA, Yahoo, Numenta, Amazon, Twitter, and on a dataset of anomaly activities in elderly home residences. Interestingly, our findings match the intuition that anomaly can be detected in cases when the model is certain of its reconstruction, but it is mistaken.
\AF{Here we're missing the Swat dataset. Should we mention also here that tadgan was designed for univ. signals?}


% The progress in modelling time series and, more generally, sequences of structure-data has recently revamped research in anomaly detection. The task stands for identifying abnormal behaviors in financial series, IT systems, aerospace measurements, and the medical domain, where anomaly detection may aid in isolating cases of depression and attend the elderly. Anomaly detection in time series is a complex task since anomalies are rare due to highly non-linear temporal correlations and since the definition of anomalous is sometimes subjective.

% In this work, we argue for a novel approach to anomaly detection which integrates uncertainty. It follows from recent trends whereby uncertainty is key to self-supervised learning. We show that uncertainty integrates well with the current approaches to anomaly detection, mainly based on sequence reconstruction errors and out-of-distribution detection. Specifically, we consider an LSTM model trained with cycle consistency and a GAN critic for anomaly detection. We propose the hyperbolic uncertainty for anomaly detection. This yields a principled formulation of an end-to-end trainable uncertainty, which they seamlessly integrate into the anomaly detector. Altogether, our proposed model outperforms the current state-of-the-art on established anomaly benchmarks based on data from NASA, Yahoo, Numenta, Amazon, Twitter, and on a dataset of anomaly activities in elderly home residences.

%The progress in modelling time series and more generally sequences of structure-data has recently revamped research in anomaly detection. The task stands for identifying abnormal behaviors in financial series, IT systems, aerospace measurements as well as in the medical domain, where anomaly detection may aid in isolating cases of depression and attend the elderly. This is a complex task, since anomalies are rare, mostly due to highly non-linear temporal correlations, and since the definition of anomalous is sometimes subjective.

%In this work, we argue for a novel approach to anomaly detection which integrates uncertainty. This follows from recent trends whereby uncertainty is key to self-supervised learning. We show that uncertainty integrates well with the current approaches to anomaly detection, mainly based on sequence reconstruction errors and out-of-distribution detection. Specifically, we consider an LSTM model trained with cycle consistency and with a GAN critic for anomaly estimation; and we extend the technique by consideration of uncertainty, as estimated employing Monte-Carlo dropout.

%We further propose the first anomaly detection model based on hyperbolic neural networks. These are the most recent techniques, they offer a principled formulation of uncertainty that is end-to-end trainable and they seamlessly integrate into the anomaly detector. Altogether, our proposed model outperforms the current state-of-the-art on established anomaly benchmarks based on data from NASA, Yahoo, Numenta, Amazon, and Twitter, as well as on a dataset of anomaly activities in elderly home residences.


% Hence, coping with the certainty of the model prediction is of paramount importance. To utilise uncertainty efficiently in anomaly detection in time series, we propose HyperTadGAN, an unsupervised reconstruction method, to work on hyperbolic vector spaces. In this way, we can distinguish between highly-confident and low-confident predicted instances. Therefore, in our scenario, an anomaly is triggered when an event outlies the normal distribution of the data and the model is sure about its prediction.

% We predict anomalous events on well-established outlier detection univariate benchmarks and multivariate elderly daily routine trajectories. We demonstrate that our proposed method achieves better results than the state-of-the-art models on both test-beds. Finally, we compare the hyperbolic uncertainty mechanism with the traditional Monte Carlo dropout used to determine the model confidence. Besides showing that uncertainty ameliorates performances in general, we demonstrate that hyperbolic neural networks achieve better results by a large margin by better suppressing false positive and false negative errors.

\end{abstract}

==> sec/Backup/exp_bk_2022-02-10.tex <==
\section{Results}\label{sec:expres}

\subsection{Datasets, metrics, and experimentation setup}\label{sec:dataset}

\FG{shall we directly start with: "We compare HypAD against the current best univariate anomaly detector TadGAN~[ref] on a benchmark of 11 time series~[ref], and extend the comparison to 2 multivariate sensor datasets: one comprising a water treatment plant and one comprising daily activities in elderly residences." In this way, it's clear upfront what is comparable to what, fairly, and we do not need a a-posteriori justification.}
To analyse the performances of HyAD w.r.t.\ the state-of-the-art we employ several anomaly benchmarks on 11 univariate time series,\BM{1 cyber-physical system dataset}\FG{these terms are not telling me much. I'd prefer a more description "sensor data from a water treatment plant". Is the terminology "cyber-physical system" established for SWaT? If so, I won't complain :))}, and 1 medical dataset containing multivariate sensoristic data on elderly home residences \cite{cook2012casas}. 
Table \ref{tab:datasets} illustrates a summarised analysis of the main characteristics of the datasets. For each dataset, we illustrate the number of signals which represent the number of different inputs within the same category. In other words, the number of signals is the number of different time series coming from several files. Notice that we only have one signal per medical condition (e.g. Nocturia, MoreTimeInChair) in the multivariate scenario\footnote{We abbreviate the signals in CASAS: Fall (F), MoreTimeInChair (MTC), Weakness (W), SlowerWalking (SW), and Nocturia (N).}. The number of anomalies depicts the sum of the number of instances with a corresponding anomalous label. As in \cite{geiger2020tadgan}, we also observe whether the anomalies in the dataset are point or collective anomalies\footnote{A point anomaly is a single instance isolated in time that is anomalous. Whereas, a collective anomaly is constituted by multiple subsequent anomalies in time.}. \FG{any comment after the observation? may one say that point anomalies are more difficult? They occur in Yahoo, where we are outperformed. I just raise this comment here because an observation without a conclusion may be used against us.} Finally, to elucidate the hardness of the anomaly detection in each dataset, we label each anomaly point as out-of-distribution if it falls $4\sigma$ away from the mean of a particular signal \FG{is there a reference for this type of observation? It feels like this would only be valid under a Gaussian assumption?}. \FG{Among the univariate time series, -- maybe better to add it upfront, instead of commenting that this only applies to univariate, else one may straightaway complain about this statement of what is more complex} According to this labelling strategy, NASA (SMAP), and Yahoo (A1, A2) represent the hardest scenarios since the percentage of out-of-distribution instances is elevated, in some cases surpassing that of the non anomalous instances (i.e. A1). Note that this approach is meaningful for the univariate datasets, but cannot be applied in the multivariate scenario. 

\paragraph{Univariate datasets} \textit{NASA} includes two spacecraft telemetry datasets\footnote{MSL and SMAP can be downloaded from \url{https://s3-us-west-2.amazonaws.com/telemanom/data.zip}.} based on the Mars Science Laboratory (MSL) and the Soil Moisture Active Passive (SMAP) signals. The former consists of scientific and housekeeping engineering data taken from the Rover Environmental Monitoring Station aboard the Mars Science Laboratory. The latter includes measurements of soil moisture and freeze/thaw state from space for all non-liquid water surfaces globally within the top layer of the Earth.


We analyse \textit{Yahoo} datasets based on real production traffic to Yahoo computing systems. Additionally, we consider three synthetic datasets coming from the same source\footnote{Upon request, the dataset can be downloaded from \url{https://webscope.sandbox.yahoo.com/catalog.php?datatype=s&did=70}}. The dataset tests the detection accuracy of various anomaly-types including outliers and change-points. The synthetic dataset consists of time-series with varying trend, noise and seasonality. The real dataset consists of time-series representing the metrics of various Yahoo services.

\textit{Numenta Anomaly Benchmark (NAB)} is a well-established collection of univariate time-series from real-world application domains\footnote{We invite the reader to consult \url{https://github.com/numenta/NAB/tree/master/data} for the entire directory of datasets.}. To be consistent with \cite{geiger2020tadgan}, we analyse Art, AdEx, AWS, Traf, and Tweets from the original collection.
   


\paragraph{Multivariate dataset} We consider \BM{for analysis the SWaT~\cite{10.1007/978-3-319-71368-7_8,Mathur2016SWaTAW} and CASAS~\cite{cook2012casas,dahmen2021indirectly} datasets.

\noindent \textit{SWaT} is collected from a cyber-physical system testbed that is a scaled down replica of an industrial water treatment plant. The data was collected every second for a total of 11 days, where for the first few days the system was operated normally, while for the remaining days certain cyber-physical attacks were launched. Following~\cite{10.1145/3447548.3467137}, we sampled sensor data every every five seconds.} 

\noindent \textit{CASAS} is a collection of two weeks of sensor data from retirement homes. Each sensor reading has a label attached according to the activity recognised by human annotators. In this way, we have a collection of time series of activities performed by elderly people. Furthermore, the anomalies are labelled according to several medical conditions\footnote{Because most of the people involved in the test suffer from chronic diseases such as severe depression and Alzheimer's, criteria like falling, night toilet visits, weakness in performing activities are used to label the time series.} established prior to the experimentation. Although sensor readings give fine-grained information, we are interested in creating daily patient profiles. Hence, we collapse them into a single engendered activity with a start and end time\footnote{The start time corresponds to the first sensor reading for that activity, whereas the end time is the last reading.} for each consecutive sensor signal. We then create a time matrix structure $\mathcal{M}^{|d|,1440}$ where $|d|$ is the number of days the patient is monitored and 1440 represent the total number of minutes in a day. $\mathcal{M}[i,j]$ represents the label performed in minute $j$ of day $i$. Lastly, we densify each value $\mathcal{M}[i,j]$ with contextual and duration information corresponding to the label therein. 

Finally, we create train and test splits of this data, caring to safeguard sequentiality of observations, and gathering the few anomalies into the test set for evaluation only. For this reason we name this Unsupervised-CASAS, dubbed U-CASAS, differing from the original CASAS \cite{cook2012casas,dahmen2021indirectly} since the latter interleaves anomalous sensor readings with normal instances, thus breaking the sequentiality of anomalies.
%IMPORTANT: later in the results mention that the ranking of methods are the same as in [??], maybe, but one cannot test isudra due to being supervised -- need to better say why we do not test against those proposing it .
For each anomalous day encountered in the test set, we pad two days prior to it and two after. If the padding overlaps with another anomalous day, then we concatenate\footnote{The concatenation procedure merges common sequences. If the sequence contains more than one anomalous day within the two-day padding window, the padded sequence gets collapsed into a single one.} them and perform the padding procedure again. We delete the days assigned to the test set from the overall dataset and assign the rest as training. Moreover, because we employ a time-related strategy, we create time windows of 30 actions to detect anomalies.




\paragraph{Metrics}
Being all the enlisted datasets highly unbalanced, accuracy is misleading. Therefore, as done in \cite{suris2021hyperfuture},we use the F1 score to account for this challenge. Based on \cite{hundman2018detecting}, we penalise high false positive rates and encourage the detection of true positive in a timely fashion. Since anomalies are rare events and come in collective sequences in real-world applications, we proceed as follows:
\begin{enumerate} %[noitemsep,topsep=0pt] 
\item We record a true positive (TP) if any predicted window overlaps a true anomalous window.
\item We record a false negative (FN) if a true anomalous window does not overlap any predicted window.
\item We record a false positive (FP) if a predicted window does not overlap any true anomalous region.
\end{enumerate}
For U-CASAS, we also measure the g-measure which is the geometric mean of the product of recall (R) and precision (P), being a robust metric when classes are imbalanced \cite{dahmen2021indirectly}.

\input{tab/performances_univariate}
\input{tab/performances_casas}

\paragraph{Baselines}
 We include the following strategies as our baselines in this paper:
\begin{itemize} %[noitemsep,topsep=0pt]
    \item \textit{AE} \cite{baldi2012autoencoders} - We use a six-layer fully-connected autoencoder.
    \item \textit{ConvAE} \cite{maggipinto2018convolutional} - We have three layers of convolutional encoding interleaved with max pooling. The decoder has a specular composition as the encoder where the de-convolution is aided by two-dimensional up-sampling layers.
    \item \textit{LstmAE} \cite{sagheer2019unsupervised} - We use a deep stacked LSTM autoencoder with four layers. The first LSTM hidden and output vectors get passed to the second LSTM layer. The latent representation of the encoder gets then reconstructed in reverse order from the decoder.
    \item \textit{TadGAN*} \cite{geiger2020tadgan} - We use a one-layer bidirectional LSTM for the generator $E$, and a two-layer bidirectional LSTM for $G$. For the critic $D_z$ we use a fully connected layer, and two dense layers for $D_x$.
\end{itemize}


\noindent\textit{Implementation details.} For the first three baselines, we set the number of epochs to 30, the batch size to 32, and the learning rate to $10^{-3}$. For TadGAN*, we set the epochs to 30, the batch size to 64, the learning rate to $5\times10^{-4}$, and the iteration for the critic to 5. We use Adam as the optimisation function to train all the baselines. 


%\BM{For the four baselines, we follow the implementation details in \cite{baldi2012autoencoders}, \cite{maggipinto2018convolutional}, \cite{sagheer2019unsupervised} and \cite{geiger2020tadgan}, respectively. For HypAD, we took inspiration ..} 

For our proposed method HypAD, we took inspiration from an online available PyTorch implementation\footnote{\url{https://github.com/arunppsg/TadGAN}}. We leave the architecture of TadGAN unvaried, but we incorporate the hyperbolic transformation\footnote{\url{https://github.com/cvlab-columbia/hyperfuture}} as in \cite{suris2021hyperfuture}. The hyperparameters are the same in the original paper, but we use the Riemannian Adam\footnote{\url{https://github.com/geoopt/geoopt}} as optimisation function.


%We set the epochs to 30, the batch size to 64, the learning rate to $5e-4$, and the iteration for the critic to 5. 
%\BM{The hyper-parameters look same as TadGAN*, may be we can remove the line before and say "The hyper-paramters are same as TadGAN* but we use the Riemannian Adam as optimisation function."}
%We use the Riemannian Adam\footnote{\url{https://github.com/geoopt/geoopt}} as optimisation function.



%\begin{itemize}[noitemsep,topsep=0pt]
%    \item \textit{AE} \cite{baldi2012autoencoders} - We use a six-layer fully-connected autoencoder. The number of neurons employed are 32, 16, and 8, respectively, for each layer of the encoder. The decoder reconstructs the bottleneck in reverse order. We use ReLU as activation function.
%    \item \textit{ConvAE} - We have three layers of convolutional encoding with 64, 32, and 16 filters, respectively. We use a $2\times 2$ kernel for each convolution layer with same padding and stride equal to 1. The decoder has a specular composition as the encoder where the de-convolution is aided by two-dimensional up-sampling layers\footnote{We refer the reader to \url{https://keras.io/api/layers/reshaping_layers/up_sampling2d/} for the adopted up-sampling technique.}. The activation function for each layer is ReLU.
%    \item \textit{LstmAE} - The encoder has two layers of LSTMs with 32 and 16 units, respectively. The decoder is specular. Each layer relies on ReLU as activation function.
%    \item \textit{TadGAN*} - As in the original paper~\cite{geiger2020tadgan}, the latent space of TadGAN* has 20 dimensions. We use a one-layer bidirectional LSTM with 100 hidden units for the generator $E$, and a two-layer bidirectional LSTM with 64 hidden units as the generator $G$. In $G$ we also apply dropout. Finally, we add one fully connected layer with 1 output neuron for the Critic $D_z$, and two dense layers with 20 and 1 output neuron, respectively, for the Critic $D_x$.
%\end{itemize}


\subsection{Comparison to the state of the art}
\textbf{HypAD outperforms all the baseline methods by
having the highest average F1-scores of 0.631 and 0.428 across the univariate and multivariate datasets, respectively.} Both Tables \ref{tab:performances_univariate} and \ref{tab:performances_casas} rank all the methods based on their averaged F1 scores (the last column) across all datasets. HypAD outperforms the second (TadGAN*, 0.600) and the third (ConvAE, 0.212) by 5.17\% and 197.64\%, respectively in the univariate scenario. Contrarily, HypAD surpasses TadGAN* by 32.51\% and ConvAE by 486.3\% according to the averaged F1-score, in the multivariate scenario.

Table \ref{tab:performances_univariate} depicts the comparison of our proposed method, HypAD, with the baselines strategies described above. For reference purposes, we enlist also the performances of TadGAN as reported\footnote{We implemented TadGAN relying on PyTorch which does not match the reported performances in the original paper.} in \cite{geiger2020tadgan}. Here, we report the F1-score, and the mean and standard deviation over all datasets. Notice that only TadGAN competes with HypAD. In this scenario, we have time windows of 100 values. Because we apply the poincaré distance directly on the windows and not on the reconstructed signal as with TadGAN, HypAD experiences a slight drop in performances. Nevertheless, with an average F1-score of $0.631$, HypAD is the best-performing method in the univariate case.

Table \ref{tab:performances_casas} illustrates the performances in the multivariate scenario \BM{on the U-CASAS dataset}. We cannot  include Isudra\cite{dahmen2021indirectly} because the underlying architecture uses a small amount of labels to conduct the selection of parameters for the execution. Additionally, Isudra is trained in a supervised fashion differing from all the other methods reported here. However, for completeness purposes, we also report the g-measure and its average across all datasets. Here, the dominance of HypAD is more evident since the transformation of multivariate time window in hyperspace has the benefit of learning latent relationships between the input features. Notice that HypAD is the best-performing method according to both g-measure and F1-score.

\BM{Table \ref{tab:performances_swat_fg} compares the proposed HypAD to other methods on the SWaT dataset. Following previous works~\cite{10.1145/3447548.3467137}, we also report the precision and recall in addition to the F1- score. As shown in the table, HypAD gives the highest precision (0.996) among all other methods. This means thate our model detects an anomaly only when it is certain of its understanding of the input signal and therefore refrains from giving wrong anomalies. However, HypAD still lags behind the other recent approaches in terms of recall and F1-score. We argue that..  } 


\input{tab/swat_permormances}

\input{tab/ablation}
% \input{tab/ablation_univariate}
% \input{tab/ablation_multivariate}
\subsection{Ablation Studies}
\BM{In Table~\ref{tab:ablation}, we demonstrate the effectiveness of HypAD on three different dataset types: Univariate, U-CASES and SWaT. The first row shows the performance of the model in euclidean space. This corresponds to the model TadGAN* in Table~\ref{tab:performances_univariate},~\ref{tab:performances_casas} and~\ref{tab:performances_swat_fg}. Next we move the model to the hyperbolic space as discussed in Section~\ref{sec:hypRe}. This brings an improvement of 0.7\% and 18.6\% in the F1 score for the univariate and U-CASES datasets, respectively. However for the SWaT  dataset the performance drops, which we discuss qualitatively in the following section. Finally, we integrate the hyperbolic uncertainty to the anomaly detection. As shown in the last two rows of the table, this brings an improvement of 4.5\% (0.604 vs 0.631) for the univariate cases, 7.8\% (0.397 vs 0.428) for the U-CASES and 33\% for the SWaT. Clearly, \textbf{Uncertainty is fundamental in ameliorating anomaly detection.} For all the datasets, the best performance is achieved using the proposed hyperbolic uncertainty.}
 
\noindent \textbf{Qualitative Ablation on SWaT:} \BM{In Figure \ref{fig:ablation1}, we demonstrate qualitative ablation on SWaT dataset that consists of only one long-term signal. The three plots correspond to the three rows in the last column of Table~\ref{tab:ablation}. In all plots, the blue and green points represent the predicted anomaly scores and ground-truth anomalies, respectively. The red line denotes the anomaly detection threshold i.e. the blue points that lie above the red line are predicted anomalies. If a blue point lies above the red line but does not coincide with any green point (ground-truth), it is a false positive.

As visible in the Figure, the model in euclidean space (first plot) gives a lot of false positives but when moving to hyperbolic space (second plot) the model becomes more precise reducing false positives substantially. However note that this hyperbolic model also brings a part of positive anomalies (in the middle of the signal) below the threshold, reducing true positives. This explains the drop in the F-1 score for the SWaT dataset (cf. Table \ref{tab:ablation}). Interestingly, the integration of uncertainty recovers these points back in addition to others, increasing the true positives but not false positives, giving the best F-1 score of 0.753.}



%which is marked as red when it is above the anomaly detection threshold. That is, the red points denotes the predicted anomalies of the model. 
%\input{fig/ablation.tex}
\input{fig/ablation1.tex}




%We evaluate multiple variations of HypAD, using different anomaly score computation methods. Tables \ref{tab:ablation_univariate} and \ref{tab:ablation_multivariate} summarise the performances of each variant. 
%Table \ref{tab:ablation_univariate} reports the average F1 score across the univariate datasets. As shown in the first two rows of the table, the integration of hyperbolic uncertainty to the reconstruction-based anomaly detection brings an improvement of 3\% (0.574 vs 0.592).  Similarly, hyperbolic uncertainty brings an improvement of 4.5\% on the combination of reconstruction error and critic score (0.604 vs 0.631), as shown in the last two rows of the table. 

%In Table \ref{tab:ablation_multivariate}, we report the average F1 score and g-measure for the multivariate case. As shown in the first two rows of the table, the hyperbolic uncertainty jointly with the reconstruction component brings an improvement of 3.4\% in terms of F1 score, 10.7\% according to the g-measure. Similarly, using it with the combination of  reconstruction error and critic score brings improvement of 7.8\% in the F1 score and 4.6\% in the g-measure.

%Clearly, for both the univariate and multivariate datasets, the best performance is achieved using all three measures: i.e. reconstruction error, critic score and uncertainty, which is the idea behind HypAD.   













==> sec/Backup/exp_bk_2022-02-11.tex <==
\section{Results}\label{sec:expres}

We compare HypAD against the current best univariate anomaly detector TadGAN~\cite{geiger2020tadgan} on a benchmark of 11 time series, and extend the comparison to 2 multivariate sensor datasets: one comprising a water treatment plant and one comprising daily activities in elderly residences.
First, we introduce the benchmarks (Sec.~\ref{sec:dataset}), then we compare against baselines and the state-of-the-art (Sec.~\ref{sec:sota}), finally we conduct ablative studies on the importance of uncertainty for performance and the reduction of false alarms (Sec.~\ref{sec:abl}).



\subsection{Datasets, metrics, and experimentation setup}\label{sec:dataset}

Table \ref{tab:datasets} illustrates a summarised analysis of the main characteristics of the datasets. For each dataset, we illustrate the number of signals which represent the number of different inputs within the same category. In other words, the number of signals is the number of different time series coming from several files. Notice that we only have one signal per medical condition (e.g. Nocturia, MoreTimeInChair) in the multivariate scenario\footnote{We abbreviate the signals in CASAS: Fall (F), MoreTimeInChair (MTC), Weakness (W), SlowerWalking (SW), and Nocturia (N).}. The number of anomalies depicts the sum of the number of instances with a corresponding anomalous label. As in \cite{geiger2020tadgan}, we also observe whether the anomalies in the dataset are point or collective anomalies\footnote{A point anomaly is a single instance isolated in time that is anomalous. Whereas, a collective anomaly is constituted by multiple subsequent anomalies in time.}. \FG{any comment after the observation? may one say that point anomalies are more difficult? They occur in Yahoo, where we are outperformed. I just raise this comment here because an observation without a conclusion may be used against us.} Finally, to elucidate the hardness of the anomaly detection in each dataset, we label each anomaly point as out-of-distribution if it falls $4\sigma$ away from the mean of a particular signal. \FG{is there a reference for this type of observation? It feels like this would only be valid under a Gaussian assumption?}. \FG{Among the univariate time series, -- maybe better to add it upfront, instead of commenting that this only applies to univariate, else one may straightaway complain about this statement of what is more complex} According to this labelling strategy, NASA (SMAP), and Yahoo (A1, A2) represent the hardest scenarios since the percentage of out-of-distribution instances is elevated, in some cases surpassing that of the non anomalous instances (i.e. A1). Note that this approach is meaningful for the univariate datasets, but cannot be applied in the multivariate scenario. 

\paragraph{Univariate datasets} \textit{NASA} includes two spacecraft telemetry datasets\footnote{MSL and SMAP can be downloaded from \url{https://s3-us-west-2.amazonaws.com/telemanom/data.zip}.} based on the Mars Science Laboratory (MSL) and the Soil Moisture Active Passive (SMAP) signals. The former consists of scientific and housekeeping engineering data taken from the Rover Environmental Monitoring Station aboard the Mars Science Laboratory. The latter includes measurements of soil moisture and freeze/thaw state from space for all non-liquid water surfaces globally within the top layer of the Earth.


We analyse \textit{Yahoo} datasets based on real production traffic to Yahoo computing systems. Additionally, we consider three synthetic datasets coming from the same source\footnote{Upon request, the dataset can be downloaded from \url{https://webscope.sandbox.yahoo.com/catalog.php?datatype=s&did=70}}. The dataset tests the detection accuracy of various anomaly-types including outliers and change-points. The synthetic dataset consists of time-series with varying trend, noise and seasonality. The real dataset consists of time-series representing the metrics of various Yahoo services.

\textit{Numenta Anomaly Benchmark (NAB)} is a well-established collection of univariate time-series from real-world application domains\footnote{We invite the reader to consult \url{https://github.com/numenta/NAB/tree/master/data} for the entire directory of datasets.}. To be consistent with \cite{geiger2020tadgan}, we analyse Art, AdEx, AWS, Traf, and Tweets from the original collection.
   


\paragraph{Multivariate dataset} We consider for analysis the SWaT~\cite{10.1007/978-3-319-71368-7_8,Mathur2016SWaTAW} and CASAS~\cite{cook2012casas,dahmen2021indirectly} datasets.

\noindent \textit{SWaT} is collected from a cyber-physical system testbed that is a scaled down replica of an industrial water treatment plant. The data was collected every second for a total of 11 days, where for the first few days the system was operated normally, while for the remaining days certain cyber-physical attacks were launched. Following~\cite{10.1145/3447548.3467137}, we sampled sensor data every every 5 seconds.

\noindent \textit{CASAS} is a collection of two weeks of sensor data from retirement homes. Each sensor reading has a label attached according to the activity recognised by human annotators. In this way, we have a collection of time series of activities performed by elderly people. Furthermore, the anomalies are labelled according to several medical conditions\footnote{Because most of the people involved in the test suffer from chronic diseases such as severe depression and Alzheimer's, criteria like falling, night toilet visits, weakness in performing activities are used to label the time series.} established prior to the experimentation. Although sensor readings give fine-grained information, we are interested in creating daily patient profiles. Hence, we collapse them into a single engendered activity with a start and end time\footnote{The start time corresponds to the first sensor reading for that activity, whereas the end time is the last reading.} for each consecutive sensor signal. We then create a time matrix structure $\mathcal{M}^{|d|,1440}$ where $|d|$ is the number of days the patient is monitored and 1440 represent the total number of minutes in a day. $\mathcal{M}[i,j]$ represents the label performed in minute $j$ of day $i$. Lastly, we densify each value $\mathcal{M}[i,j]$ with contextual and duration information corresponding to the label therein. 

Finally, we create train and test splits of this data, caring to safeguard sequentiality of observations, and gathering the few anomalies into the test set for evaluation only. For this reason we name this Unsupervised-CASAS, dubbed U-CASAS, differing from the original CASAS \cite{cook2012casas,dahmen2021indirectly} since the latter interleaves anomalous sensor readings with normal instances, thus breaking the sequentiality of anomalies.
%IMPORTANT: later in the results mention that the ranking of methods are the same as in [??], maybe, but one cannot test isudra due to being supervised -- need to better say why we do not test against those proposing it .
For each anomalous day encountered in the test set, we pad two days prior to it and two after. If the padding overlaps with another anomalous day, then we concatenate\footnote{The concatenation procedure merges common sequences. If the sequence contains more than one anomalous day within the two-day padding window, the padded sequence gets collapsed into a single one.} them and perform the padding procedure again. We delete the days assigned to the test set from the overall dataset and assign the rest as training. Moreover, because we employ a time-related strategy, we create time windows of 30 actions to detect anomalies.



\paragraph{Metrics}
Being all the enlisted datasets highly unbalanced, accuracy is misleading. Therefore, as done in \cite{suris2021hyperfuture},we use the F1 score to account for this challenge. Based on \cite{hundman2018detecting}, for the univariate and the CASAS datasets, we penalize high false positive rates and encourage the detection of true positive in a timely fashion. Since anomalies are rare events and come in collective sequences in real-world applications, we proceed as follows:
\begin{enumerate} %[noitemsep,topsep=0pt] 
\item We record a true positive (TP) if any predicted window overlaps a true anomalous window.
\item We record a false negative (FN) if a true anomalous window does not overlap any predicted window.
\item We record a false positive (FP) if a predicted window does not overlap any true anomalous region.
\end{enumerate}
For U-CASAS, we also measure the g-measure which is the geometric mean of the product of recall (R) and precision (P), being a robust metric when classes are imbalanced \cite{dahmen2021indirectly}.

\input{tab/performances_univariate}
\input{tab/performances_casas}

\paragraph{Baselines}
 We include the following strategies as our baselines in this paper:
\begin{itemize} %[noitemsep,topsep=0pt]
    \item \textit{AE} \cite{baldi2012autoencoders} - We use a six-layer fully-connected autoencoder.
    \item \textit{ConvAE} \cite{maggipinto2018convolutional} - We have three layers of convolutional encoding interleaved with max pooling. The decoder has a specular composition as the encoder where the de-convolution is aided by two-dimensional up-sampling layers.
    \item \textit{LstmAE} \cite{sagheer2019unsupervised} - We use a deep stacked LSTM autoencoder with four layers. The first LSTM hidden and output vectors get passed to the second LSTM layer. The latent representation of the encoder gets then reconstructed in reverse order from the decoder.
    \item \textit{TadGAN*} \cite{geiger2020tadgan} - We use a one-layer bidirectional LSTM for the generator $E$, and a two-layer bidirectional LSTM for $G$. For the critic $D_z$ we use a fully connected layer, and two dense layers for $D_x$.
\end{itemize}


\noindent\textit{Implementation details.} For the first three baselines, we set the number of epochs to 30, the batch size to 32, and the learning rate to $10^{-3}$. For TadGAN*, we set the epochs to 30, the batch size to 64, the learning rate to $5\times10^{-4}$, and the iteration for the critic to 5. We use Adam as the optimisation function to train all the baselines. 


%\BM{For the four baselines, we follow the implementation details in \cite{baldi2012autoencoders}, \cite{maggipinto2018convolutional}, \cite{sagheer2019unsupervised} and \cite{geiger2020tadgan}, respectively. For HypAD, we took inspiration ..} 

For our proposed method HypAD, we took inspiration from an online available PyTorch implementation\footnote{\url{https://github.com/arunppsg/TadGAN}}. We leave the architecture of TadGAN unvaried, but we incorporate the hyperbolic transformation\footnote{\url{https://github.com/cvlab-columbia/hyperfuture}} as in \cite{suris2021hyperfuture}. The hyperparameters are the same in the original paper, but we use the Riemannian Adam\footnote{\url{https://github.com/geoopt/geoopt}} as optimisation function.


%We set the epochs to 30, the batch size to 64, the learning rate to $5e-4$, and the iteration for the critic to 5. 
%\BM{The hyper-parameters look same as TadGAN*, may be we can remove the line before and say "The hyper-paramters are same as TadGAN* but we use the Riemannian Adam as optimisation function."}
%We use the Riemannian Adam\footnote{\url{https://github.com/geoopt/geoopt}} as optimisation function.



%\begin{itemize}[noitemsep,topsep=0pt]
%    \item \textit{AE} \cite{baldi2012autoencoders} - We use a six-layer fully-connected autoencoder. The number of neurons employed are 32, 16, and 8, respectively, for each layer of the encoder. The decoder reconstructs the bottleneck in reverse order. We use ReLU as activation function.
%    \item \textit{ConvAE} - We have three layers of convolutional encoding with 64, 32, and 16 filters, respectively. We use a $2\times 2$ kernel for each convolution layer with same padding and stride equal to 1. The decoder has a specular composition as the encoder where the de-convolution is aided by two-dimensional up-sampling layers\footnote{We refer the reader to \url{https://keras.io/api/layers/reshaping_layers/up_sampling2d/} for the adopted up-sampling technique.}. The activation function for each layer is ReLU.
%    \item \textit{LstmAE} - The encoder has two layers of LSTMs with 32 and 16 units, respectively. The decoder is specular. Each layer relies on ReLU as activation function.
%    \item \textit{TadGAN*} - As in the original paper~\cite{geiger2020tadgan}, the latent space of TadGAN* has 20 dimensions. We use a one-layer bidirectional LSTM with 100 hidden units for the generator $E$, and a two-layer bidirectional LSTM with 64 hidden units as the generator $G$. In $G$ we also apply dropout. Finally, we add one fully connected layer with 1 output neuron for the Critic $D_z$, and two dense layers with 20 and 1 output neuron, respectively, for the Critic $D_x$.
%\end{itemize}


\subsection{Comparison to the state of the art} \label{sec:sota}


\textbf{HypAD defines a new state-of-the-art performance for univariate anomaly detection by having the highest average F1-scores of 0.631.} 
\FG{Please split this statement. Leave here only the univariate, else our earlier note is spoiled. I mean: it's best to discuss univariate, and then say that we extend this test to multivariate.} 
Both Tables \ref{tab:performances_univariate} and \ref{tab:performances_casas} rank all the methods based on their averaged F1 scores (the last column) across all datasets. HypAD outperforms the second (TadGAN*, 0.600) and the third (ConvAE, 0.212) by 5.17\% and 197.64\%, respectively in the univariate scenario. Contrarily, HypAD surpasses TadGAN* by 32.51\% and ConvAE by 486.3\% according to the averaged F1-score, in the multivariate scenario. 
\FG{in the spirit of my note, please check that all earlier paragraphs regard univariate just.}

Table \ref{tab:performances_univariate} depicts the comparison of our proposed method, HypAD, with the baselines strategies described above. For reference purposes, we enlist also the performances of TadGAN as reported\footnote{We implemented TadGAN relying on PyTorch which does not match the reported performances in the original paper.} in \cite{geiger2020tadgan}. Here, we report the F1-score, and the mean and standard deviation over all datasets. Notice that only TadGAN competes with HypAD. In this scenario, we have time windows of 100 values. Because we apply the poincaré distance directly on the windows and not on the reconstructed signal as with TadGAN, HypAD experiences a slight drop in performances. Nevertheless, with an average F1-score of $0.631$, HypAD is the best-performing method in the univariate case.

In Table~\ref{tab:performances_casas} we extend the evaluation of HypAD to the multivariate scenario of the U-CASAS dataset. We cannot  include Isudra\cite{dahmen2021indirectly} because the underlying architecture uses a small amount of labels to conduct the selection of parameters for the execution. Additionally, Isudra is trained in a supervised fashion differing from all the other methods reported here. However, for completeness purposes, we also report the g-measure and its average across all datasets. Here, the dominance of HypAD is more evident since the transformation of multivariate time window in hyperspace has the benefit of learning latent relationships between the input features. Notice that HypAD is the best-performing method according to both g-measure and F1-score. 
\FG{I'd suggest smoothing this message, else it seems one should expect higher performance from multivariate, which is not the case.}

Finally, in Table~\ref{tab:performances_swat_fg}, we also extend comparison to the multivariate SWaT dataset. Here, following previous work~\cite{10.1145/3447548.3467137}, we also report the precision and recall in addition to the F1-score. HypAD outperforms the baseline TadGAN (0.753 Vs.\ 0.722) but both techniques are behind the current state-of-the-art on multivariate anomaly detection NSIBF~\cite{10.1145/3447548.3467137}.
Observe however that HypAD achieves its highest F1-performance at the highest precision (0.996) among all other methods. This confirms that HypAD really detects anomalies which it is certain about, i.e.\ when it \emph{understands} the time series, it is certain about what to expect, but cannot reconstruct the input signal due to an anomaly.


\input{tab/swat_permormances}

\input{tab/ablation}
% \input{tab/ablation_univariate}
% \input{tab/ablation_multivariate}



\subsection{Ablation Studies}\label{sec:abl}

In Table~\ref{tab:ablation}, we demonstrate the effectiveness of HypAD on three different dataset types: Univariate, U-CASAS and SWaT. The first row shows the performance of the model in euclidean space. This corresponds to the model TadGAN* in Table~\ref{tab:performances_univariate},~\ref{tab:performances_casas} and~\ref{tab:performances_swat_fg}. Next we move the model to the hyperbolic space as discussed in Section~\ref{sec:hypRe}. This brings an improvement of 0.7\% and 18.6\% in the F1 score for the univariate and U-CASAS datasets, respectively. However for the SWaT  dataset the performance drops, which we discuss qualitatively in the following section. Finally, we integrate the hyperbolic uncertainty to the anomaly detection. As shown in the last two rows of the table, this brings an improvement of 4.5\% (0.604 vs 0.631) for the univariate cases, 7.8\% (0.397 vs 0.428) for the U-CASAS and 33\% for the SWaT. Clearly, \textbf{Uncertainty is fundamental in ameliorating anomaly detection.} For all the datasets, the best performance is achieved using the proposed hyperbolic uncertainty.
 
\noindent \textbf{Qualitative Ablation on SWaT:} In Figure \ref{fig:ablation1}, we demonstrate qualitative ablation on the SWaT dataset that consists of only one long-term signal. The three plots correspond to the three rows in the last column of Table~\ref{tab:ablation}. In all plots, the blue and green points represent the predicted anomaly scores and ground-truth anomalies, respectively. The red line denotes the anomaly detection threshold i.e. the blue points that lie above the red line are predicted anomalies. If a blue point lies above the red line but does not coincide with any green point (ground-truth), it is a false positive.

As visible in the Figure, the model in euclidean space (first plot) gives a lot of false positives but when moving to hyperbolic space (second plot) the model becomes more precise reducing false positives substantially. However note that this hyperbolic model also brings a part of positive anomalies (in the middle of the signal) below the threshold, reducing true positives. This explains the drop in the F-1 score for the SWaT dataset (cf. Table \ref{tab:ablation}). Interestingly, the integration of uncertainty recovers these points back in addition to others, increasing the true positives but not false positives, giving the best F-1 score of 0.753.



%which is marked as red when it is above the anomaly detection threshold. That is, the red points denotes the predicted anomalies of the model. 
%\input{fig/ablation.tex}
\input{fig/ablation1.tex}




%We evaluate multiple variations of HypAD, using different anomaly score computation methods. Tables \ref{tab:ablation_univariate} and \ref{tab:ablation_multivariate} summarise the performances of each variant. 
%Table \ref{tab:ablation_univariate} reports the average F1 score across the univariate datasets. As shown in the first two rows of the table, the integration of hyperbolic uncertainty to the reconstruction-based anomaly detection brings an improvement of 3\% (0.574 vs 0.592).  Similarly, hyperbolic uncertainty brings an improvement of 4.5\% on the combination of reconstruction error and critic score (0.604 vs 0.631), as shown in the last two rows of the table. 

%In Table \ref{tab:ablation_multivariate}, we report the average F1 score and g-measure for the multivariate case. As shown in the first two rows of the table, the hyperbolic uncertainty jointly with the reconstruction component brings an improvement of 3.4\% in terms of F1 score, 10.7\% according to the g-measure. Similarly, using it with the combination of  reconstruction error and critic score brings improvement of 7.8\% in the F1 score and 4.6\% in the g-measure.

%Clearly, for both the univariate and multivariate datasets, the best performance is achieved using all three measures: i.e. reconstruction error, critic score and uncertainty, which is the idea behind HypAD.   













==> sec/Backup/exp_bk_2022-02-11b.tex <==
\section{Results}\label{sec:expres}

We compare HypAD against the current best univariate anomaly detector TadGAN~\cite{geiger2020tadgan} on a benchmark of 11 time series, and extend the comparison to 2 multivariate sensor datasets: one comprising a water treatment plant and one comprising daily activities in elderly residences.
First, we introduce the benchmarks (Sec.~\ref{sec:dataset}), then we compare against baselines and the state-of-the-art (Sec.~\ref{sec:sota}), finally we conduct ablative studies on the importance of uncertainty for performance and the reduction of false alarms (Sec.~\ref{sec:abl}).



\subsection{Datasets, metrics and experimental setup}\label{sec:dataset}

Table~\ref{tab:datasets} summarizes the main characteristics of the datasets, which we coarsely divide into univariate, main test bed of our baseline TadGAN~\cite{geiger2020tadgan}, and multivariate, to which we extend comparison. In the table, we report the sources of signals (NASA, Yahoo, NAB, CASAS and SWaT) and the datasets within each source (SMAP, MSL, A1 etc.), cf.\ detailed description later in the section.

In the table, the \textit{number of signals} is the number of time series within the datasets. Note that univariate datasets are composed of multiple signals, while the multivariate only comprise single large time series.
The \textit{number of anomalies} counts the instances, within the time series, labelled as anomalous. These are further detailed as \textit{point anomalies}, single anomalous values at a specific point in time, or \textit{collective anomalies}, sets of contiguous times which are altogether anomalous. Yahoo is the sole dataset with point anomalies, and the only with \textit{synthetic} sequences A2, A3, A4.
We also report the \textit{percentage of total} anomalous points and, following \cite{geiger2020tadgan}, for the univariate datasets, the \textit{number of out-of-distribution} points, exceeding the means by more than $4\sigma$.
% According to this labelling strategy, NASA (SMAP), and Yahoo (A1, A2) represent the hardest scenarios since the percentage of out-of-distribution instances is elevated, in some cases surpassing that of the non anomalous instances (i.e. A1). Note that this approach is meaningful for the univariate datasets, but cannot be applied in the multivariate scenario. 



\paragraph{Univariate datasets} \textit{NASA} includes two spacecraft telemetry datasets\footnote{\url{https://s3-us-west-2.amazonaws.com/telemanom/data.zip}.} based on the Mars Science Laboratory (MSL) and the Soil Moisture Active Passive (SMAP) signals. The former consists of scientific and housekeeping engineering data taken from the Rover Environmental Monitoring Station aboard the Mars Science Laboratory. The latter includes measurements of soil moisture and freeze/thaw state from space for all non-liquid water surfaces globally within the top layer of the Earth.


We analyse \textit{Yahoo} datasets based on real production traffic to Yahoo computing systems. Additionally, we consider three synthetic datasets coming from the same source\footnote{\url{https://webscope.sandbox.yahoo.com/catalog.php?datatype=s&did=70}}. The dataset tests the detection accuracy of various anomaly-types including outliers and change-points. The synthetic dataset consists of time-series with varying trend, noise and seasonality. The real dataset consists of time-series representing the metrics of various Yahoo services.

\textit{Numenta Anomaly Benchmark (NAB)} is a well-established collection of univariate time-series from real-world application domains\footnote{We invite the reader to consult \url{https://github.com/numenta/NAB/tree/master/data} for the entire directory of datasets.}. To be consistent with \cite{geiger2020tadgan}, we analyse Art, AdEx, AWS, Traf, and Tweets from the original collection.
   


 \paragraph{Multivariate datasets.} We consider for analysis the SWaT~\cite{10.1007/978-3-319-71368-7_8,Mathur2016SWaTAW} and CASAS~\cite{cook2012casas,dahmen2021indirectly} datasets.
\textit{SWaT} is collected from a cyber-physical system testbed that is a scaled down replica of an industrial water treatment plant. The data was collected every second for a total of 11 days, where for the first few days the system was operated normally, while for the remaining days certain cyber-physical attacks were launched. Following~\cite{10.1145/3447548.3467137}, we sample sensor data every every 5 seconds.


% Notice that we only have one signal per medical condition (e.g. Nocturia, MoreTimeInChair) in the multivariate scenario\footnote{We abbreviate the signals in CASAS: Fall (F), MoreTimeInChair (MTC), Weakness (W), SlowerWalking (SW), and Nocturia (N).}.

\textit{CASAS} is a collection of two weeks of sensor data from retirement homes. Each sensor reading has a label attached to it, according to the activity of elderly people recognised by human annotators. The 5 time series are collection of activities, grouped by the medical conditions established prior to the experimentation: Falling (F), More Time in Chair (MTC), Weakness (W), Slower Walking (SW), and Nocturia (N) for nightly time visits.
Although sensor readings give fine-grained information, we are interested in creating daily patient profiles. Hence, we collapse them into a single engendered activity with a start and end time\footnote{The start time corresponds to the first sensor reading for that activity, whereas the end time is the last reading.} for each consecutive sensor signal. We then create a time matrix structure $\mathcal{M}^{|d|,1440}$ where $|d|$ is the number of days the patient is monitored and 1440 represent the total number of minutes in a day. $\mathcal{M}[i,j]$ represents the label performed in minute $j$ of day $i$. Lastly, we densify each value $\mathcal{M}[i,j]$ with contextual and duration information corresponding to the label therein. 

Finally, we create train and test splits of this data, caring to safeguard sequentiality of observations, and gathering the few anomalies into the test set for evaluation only. For this reason we name this Unsupervised-CASAS, dubbed U-CASAS, differing from the original CASAS \cite{cook2012casas,dahmen2021indirectly} since the latter interleaves anomalous sensor readings with normal instances, thus breaking the sequentiality of anomalies.
%IMPORTANT: later in the results mention that the ranking of methods are the same as in [??], maybe, but one cannot test isudra due to being supervised -- need to better say why we do not test against those proposing it .
For each anomalous day encountered in the test set, we pad two days prior to it and two after. If the padding overlaps with another anomalous day, then we concatenate\footnote{The concatenation procedure merges common sequences. If the sequence contains more than one anomalous day within the two-day padding window, the padded sequence gets collapsed into a single one.} them and perform the padding procedure again. We delete the days assigned to the test set from the overall dataset and assign the rest as training. Moreover, because we employ a time-related strategy, we create time windows of 30 actions to detect anomalies.



\paragraph{Metrics}
Being all the enlisted datasets highly unbalanced, accuracy is misleading. Therefore, as done in \cite{suris2021hyperfuture},we use the F1 score to account for this challenge. Based on \cite{hundman2018detecting}, for the univariate and the CASAS datasets, we penalize high false positive rates and encourage the detection of true positive in a timely fashion. Since anomalies are rare events and come in collective sequences in real-world applications, we proceed as follows:
\begin{enumerate} %[noitemsep,topsep=0pt] 
\item We record a true positive (TP) if any predicted window overlaps a true anomalous window.
\item We record a false negative (FN) if a true anomalous window does not overlap any predicted window.
\item We record a false positive (FP) if a predicted window does not overlap any true anomalous region.
\end{enumerate}
For U-CASAS, we also measure the g-measure which is the geometric mean of the product of recall (R) and precision (P), being a robust metric when classes are imbalanced \cite{dahmen2021indirectly}.

\input{tab/performances_univariate}
\input{tab/performances_casas}

\paragraph{Baselines}
 We include the following strategies as our baselines in this paper:
\begin{itemize} %[noitemsep,topsep=0pt]
    \item \textit{AE} \cite{baldi2012autoencoders} - We use a six-layer fully-connected autoencoder.
    \item \textit{ConvAE} \cite{maggipinto2018convolutional} - We have three layers of convolutional encoding interleaved with max pooling. The decoder has a specular composition as the encoder where the de-convolution is aided by two-dimensional up-sampling layers.
    \item \textit{LstmAE} \cite{sagheer2019unsupervised} - We use a deep stacked LSTM autoencoder with four layers. The first LSTM hidden and output vectors get passed to the second LSTM layer. The latent representation of the encoder gets then reconstructed in reverse order from the decoder.
    \item \textit{TadGAN*} \cite{geiger2020tadgan} - We use a one-layer bidirectional LSTM for the generator $E$, and a two-layer bidirectional LSTM for $G$. For the critic $D_z$ we use a fully connected layer, and two dense layers for $D_x$.
\end{itemize}


\noindent\textit{Implementation details.} For the first three baselines, we set the number of epochs to 30, the batch size to 32, and the learning rate to $10^{-3}$. For TadGAN*, we set the epochs to 30, the batch size to 64, the learning rate to $5\times10^{-4}$, and the iteration for the critic to 5. We use Adam as the optimisation function to train all the baselines. 


%\BM{For the four baselines, we follow the implementation details in \cite{baldi2012autoencoders}, \cite{maggipinto2018convolutional}, \cite{sagheer2019unsupervised} and \cite{geiger2020tadgan}, respectively. For HypAD, we took inspiration ..} 

For our proposed method HypAD, we took inspiration from an online available PyTorch implementation\footnote{\url{https://github.com/arunppsg/TadGAN}}. We leave the architecture of TadGAN unvaried, but we incorporate the hyperbolic transformation\footnote{\url{https://github.com/cvlab-columbia/hyperfuture}} as in \cite{suris2021hyperfuture}. The hyperparameters are the same in the original paper, but we use the Riemannian Adam\footnote{\url{https://github.com/geoopt/geoopt}} as optimisation function.


%We set the epochs to 30, the batch size to 64, the learning rate to $5e-4$, and the iteration for the critic to 5. 
%\BM{The hyper-parameters look same as TadGAN*, may be we can remove the line before and say "The hyper-paramters are same as TadGAN* but we use the Riemannian Adam as optimisation function."}
%We use the Riemannian Adam\footnote{\url{https://github.com/geoopt/geoopt}} as optimisation function.



%\begin{itemize}[noitemsep,topsep=0pt]
%    \item \textit{AE} \cite{baldi2012autoencoders} - We use a six-layer fully-connected autoencoder. The number of neurons employed are 32, 16, and 8, respectively, for each layer of the encoder. The decoder reconstructs the bottleneck in reverse order. We use ReLU as activation function.
%    \item \textit{ConvAE} - We have three layers of convolutional encoding with 64, 32, and 16 filters, respectively. We use a $2\times 2$ kernel for each convolution layer with same padding and stride equal to 1. The decoder has a specular composition as the encoder where the de-convolution is aided by two-dimensional up-sampling layers\footnote{We refer the reader to \url{https://keras.io/api/layers/reshaping_layers/up_sampling2d/} for the adopted up-sampling technique.}. The activation function for each layer is ReLU.
%    \item \textit{LstmAE} - The encoder has two layers of LSTMs with 32 and 16 units, respectively. The decoder is specular. Each layer relies on ReLU as activation function.
%    \item \textit{TadGAN*} - As in the original paper~\cite{geiger2020tadgan}, the latent space of TadGAN* has 20 dimensions. We use a one-layer bidirectional LSTM with 100 hidden units for the generator $E$, and a two-layer bidirectional LSTM with 64 hidden units as the generator $G$. In $G$ we also apply dropout. Finally, we add one fully connected layer with 1 output neuron for the Critic $D_z$, and two dense layers with 20 and 1 output neuron, respectively, for the Critic $D_x$.
%\end{itemize}


\subsection{Comparison to the state of the art} \label{sec:sota}




\textbf{HypAD defines a new state-of-the-art performance for univariate anomaly detection by having the highest average F1-scores of 0.631.}
As shown in Table~\ref{tab:performances_univariate}, HypAD outperforms the current best technique (TadGAN*, 0.600) by 5.17\%, as well as all baselines.
% As shown in Table~\ref{tab:performances_univariate}, HypAD outperforms the second (TadGAN*, 0.600) and the third (ConvAE, 0.212) by 5.17\% and 197.64\%, respectively.

Table \ref{tab:performances_univariate} depicts the comparison of our proposed method, HypAD, with the baselines strategies described above. For reference purposes, we enlist also the performances of TadGAN as reported\footnote{We implemented TadGAN relying on PyTorch which does not match the reported performances in the original paper.} in \cite{geiger2020tadgan}. Here, we report the F1-score, and the mean and standard deviation over all datasets. \BM{The table rank all the methods based on their averaged F1 scores (the last column) across all datasets.} Notice that only TadGAN competes with HypAD. In this scenario, we have time windows of 100 values and we apply the poincaré distance directly on the windows and not on the reconstructed signal as with TadGAN\st{, HypAD experiences a slight drop in performances}. Nevertheless, with an average F1-score of $0.631$, HypAD is the best-performing method in the univariate case.

In Table~\ref{tab:performances_casas} we extend the evaluation of HypAD to the multivariate scenario of the U-CASAS dataset. We cannot include Isudra\cite{dahmen2021indirectly} because the underlying architecture uses a small amount of labels to conduct the selection of parameters for the execution. Additionally, Isudra is trained in a supervised fashion differing from all the other methods reported here. \st{However,} for completeness purposes, we also report the g-measure and its average across all datasets. \st{Here, the dominance of HypAD is more evident since the transformation of multivariate time window in hyperspace has the benefit of learning latent relationships between the input features. Notice that HypAD is the best-performing method according to both g-measure and F1-score.} \BM{As shown, HypAD surpasses TadGAN* by 32.51\% and ConvAE by 486.3\% according to the averaged F1-score.}
%\FG{I'd suggest smoothing this message, else it seems one should expect higher performance from multivariate, which is not the case.}



Finally, in Table~\ref{tab:performances_swat_fg}, we also extend comparison to the multivariate SWaT dataset. Here, following previous work~\cite{10.1145/3447548.3467137}, we also report the precision and recall in addition to the F1-score. HypAD outperforms the baseline TadGAN* (0.753 Vs.\ 0.722) but both techniques are behind the current state-of-the-art on multivariate anomaly detection NSIBF~\cite{10.1145/3447548.3467137}.
Observe however that HypAD achieves its highest F1-performance at the highest precision (0.996) among all other methods. This confirms that HypAD really detects anomalies which it is certain about, i.e.\ when it \emph{understands} the time series and is certain about what to expect, but cannot reconstruct the input signal due to an anomaly.


\input{tab/swat_permormances}

\input{tab/ablation}
% \input{tab/ablation_univariate}
% \input{tab/ablation_multivariate}



\subsection{Ablation Studies}\label{sec:abl}

In Table~\ref{tab:ablation}, we demonstrate the effectiveness of HypAD on three different dataset types: Univariate, U-CASAS and SWaT. The first row shows the performance of the model in euclidean space. This corresponds to the model TadGAN* in Table~\ref{tab:performances_univariate},~\ref{tab:performances_casas} and~\ref{tab:performances_swat_fg}. Next we move the model to the hyperbolic space as discussed in Section~\ref{sec:hypRe}. This brings an improvement of 0.7\% and 18.6\% in the F1 score for the univariate and U-CASAS datasets, respectively. However for the SWaT  dataset the performance drops, which we discuss qualitatively in the following section. Finally, we integrate the hyperbolic uncertainty to the anomaly detection. As shown in the last two rows of the table, this brings an improvement of 4.5\% (0.604 vs 0.631) for the univariate cases, 7.8\% (0.397 vs 0.428) for the U-CASAS and 33\% for the SWaT. Clearly, \textbf{Uncertainty is fundamental in ameliorating anomaly detection.} For all the datasets, the best performance is achieved using the proposed hyperbolic uncertainty.
 
\noindent \textbf{Qualitative Ablation on SWaT:} In Figure \ref{fig:ablation1}, we demonstrate qualitative ablation on the SWaT dataset that consists of only one long-term signal. The three plots correspond to the three rows in the last column of Table~\ref{tab:ablation}. In all plots, the blue and green points represent the predicted anomaly scores and ground-truth anomalies, respectively. The red line denotes the anomaly detection threshold i.e. the blue points that lie above the red line are predicted anomalies. If a blue point lies above the red line but does not coincide with any green point (ground-truth), it is a false positive.

As visible in the Figure, the model in euclidean space (first plot) gives a lot of false positives but when moving to hyperbolic space (second plot) the model becomes more precise reducing false positives substantially. However note that this hyperbolic model also brings a part of positive anomalies (in the middle of the signal) below the threshold, reducing true positives. This explains the drop in the F-1 score for the SWaT dataset (cf. Table \ref{tab:ablation}). Interestingly, the integration of uncertainty recovers these points back in addition to others, increasing the true positives but not false positives, giving the best F-1 score of 0.753.



%which is marked as red when it is above the anomaly detection threshold. That is, the red points denotes the predicted anomalies of the model. 
%\input{fig/ablation.tex}
\input{fig/ablation1.tex}




%We evaluate multiple variations of HypAD, using different anomaly score computation methods. Tables \ref{tab:ablation_univariate} and \ref{tab:ablation_multivariate} summarise the performances of each variant. 
%Table \ref{tab:ablation_univariate} reports the average F1 score across the univariate datasets. As shown in the first two rows of the table, the integration of hyperbolic uncertainty to the reconstruction-based anomaly detection brings an improvement of 3\% (0.574 vs 0.592).  Similarly, hyperbolic uncertainty brings an improvement of 4.5\% on the combination of reconstruction error and critic score (0.604 vs 0.631), as shown in the last two rows of the table. 

%In Table \ref{tab:ablation_multivariate}, we report the average F1 score and g-measure for the multivariate case. As shown in the first two rows of the table, the hyperbolic uncertainty jointly with the reconstruction component brings an improvement of 3.4\% in terms of F1 score, 10.7\% according to the g-measure. Similarly, using it with the combination of  reconstruction error and critic score brings improvement of 7.8\% in the F1 score and 4.6\% in the g-measure.

%Clearly, for both the univariate and multivariate datasets, the best performance is achieved using all three measures: i.e. reconstruction error, critic score and uncertainty, which is the idea behind HypAD.   













==> sec/Backup/intro_bk_2022-02-10.tex <==
\section{Introduction}

\input{fig/teaser}
%\AF{Comment by Alessandro.} \MAS{Comment by Marco Aurelio.} \BP{Comment by Bardh.} \BM{Comment by Bharti.} \FG{Comment by Fabio.} See the preamble file for how to use margin comments too.

%\TODO{Punch List} \FG{Place here all things remaining to be done, remove bullets when done.}
%\begin{itemize}
%    \item Make histogram on hyperbolic uncertainty
%    \item implement logistic regression on point+critic+uncertainty
%    \item re-run baselines on the new casas
%    \item Include Tables into the result section with brief explanation
%    \item Write the method part
%\end{itemize}


%\FG{We need a teaser. Please propose some.
%@alessandro: one teaser could be one of the histograms showing how anomalies occur on those reconstructions where the model is certain -- but pick one with best performance for the teaser. Another one would be to show the original (first line) Vs reconstructed (second line) signal, and show the uncertainty on a third line. But need to choose a case with high certainty on the anomaly.}

\label{sec:intro}
Anomaly detection stands for detecting outliers (anomalies) in data, i.e.\ points that deviate significantly from the distribution of the data. Outlier detection, however, is an under-specified and consequently ill-posed task due to its inherent unsupervised nature. Anomaly detection strategies such as distance-based \cite{fan2006nonparametric,ghoting2008fast}, density-based \cite{lof,papadimitriou2003loci}, and subspace-based methods \cite{keller2012hics,lazarevic2005feature} have been pioneers in the literature. Additionally, autoencoders \cite{chen2017outlier,sarvari2021unsupervised}, and adversarial networks \cite{geiger2020tadgan} have given a substantial contribution. However, the literature neglects assessing the trustfulness of the predicted outcomes, namely their uncertainty.

Uncertainty is a measure of confidence for model prediction by learning directly from the data \cite{lakshminarayanan2016simple,kendall2017uncertainties} or by having access to additional instances \cite{gal2016dropout}. Uncertainty estimation has been a long-standing challenge in machine learning. Some works based on supervised learning have exploited uncertainty approximation techniques to improve performances in scenarios such as, object detection \cite{jiang2018acquisition,kuppers2020multivariate,9156274,neumann2018relaxed}, pose estimation \cite{vakhitov2021uncertainty}, and, more complicated, scene understanding \cite{badrinarayanan2017segnet}. Recently, uncertainty has become a cardinal aspect in ameliorating the development of unsupervised/self-supervised learning approaches \cite{fiery2021,8289350,suris2021hyperfuture}. Yet it remains a largely unexplored aspect in this context. 
%Research on self-supervised learning for anomaly detection utilises generative models to estimate uncertainty excluding it in the detection \cite{li2021cutpaste,zhang2022deep,9469869} 

In this work, we propose a novel model based on Hyperbolic uncertainty for Anomaly Detection, which we dub HypAD. We leverage the current state of the art anomaly detection technique~\cite{geiger2020tadgan}, which detects anomalous events as those that are more arduous to reconstruct. The proposed hyperbolic uncertainty is integrated into the reconstruction loss according to the following modelling principle: the reconstruction loss is exponentially higher if the reconstructed signal turns out to be wrong and it was estimated with high certainty.
HypAD is therefore encouraged to reconstruct the original signal flawlessly with high certainty -- which makes the reconstruction loss zero -- or by attempting the best reconstruction with some degree of uncertainty. The latter is a self-regulating principle which is enabled by the hyperbolic Poincaré distance measure, exponentially larger for points which are certain, as we detail in Sec~\ref{sec:hypUn}.
%
%\FG{Need to introduce here our chosen algorithm for anomaly detection. My draft suggestion: "We leverage the current state of the art anomaly detection model [ref], which detects anomalous events as those that are more arduous to reconstruct.
%The reconstruction is achieved by an LSTM-based encoder, followed by a decoder, trained to match the original sequence by mean of a generative adversarial training. The proposed hyperbolic uncertainty is integrated into the reconstruction loss according to the following modelling principle: the reconstruction loss is exponentially higher if the reconstructed signal turns out to be wrong, but it was estimated with low uncertainty.HypAD is therefore encouraged to reconstruct the original signal flawlessly with high certainty -- which makes the reconstruction loss zero -- or by attempting the best reconstruction with some degree of uncertainty. The latter is a self-regulating principle which is enabled by the hyperbolic Poincare distance measure, exponentially larger for points which are certain, as we detail in Sec [ref]."In my view the remainder of this paragraph may go, please review it first.}





%Instead of using an add-on dropout layer as with MC Dropout, our strategy integrates an embedding layer to a hyperbolic vector space (hereafter \textit{hyperspace}) minimising the reconstruction error of sequences according to the Poincaré distance. Notice that the distances between the time series and their reconstructions vary when the uncertainty varies. Thus, a model uncertain of the reconstruction of a particular time series places the reconstruction at a higher uncertainty level. As a consequence, the distance between the time series and a wrongly reconstructed one is smaller if the reconstruction is uncertain, while exponentially larger if it is certain. Our model chooses, in a principled way, to mark some reconstructions as uncertain because this minimises the hyperbolic reconstruction error. An interesting and flexible approach of transforming the problem in a hyperspace is to use Hyperbolic Neural Networks \cite{NEURIPS2018_dbab2adc} - hereafter hyperNNs. They are end-to-end trainable and learn implicit hierarchical relationships of the input features by minimising a loss in hyperspace. Moreover, they have demonstrated to surpass state-of-the-art performances in next-action recognition \cite{suris2021hyperfuture} and representation learning of real-word hierarchies and scale-free graphs \cite{chami2019hyperbolic}. We additionally conduct ablation studies and show that the use of uncertainty as computer from MC dropout is also beneficial. \FG{I have place some suggestions in the earlier paragraph about topics which are explained here, now a repetition. Altogether, it feel that this paragraph should be better distinguished from the previous or removed. As a preference: I generally introduce the main take-home message in the first sentence of a paragraph. What is the message for this? I hope it's clear.}


%\FG{Need a more straightforward formulation of why hyperbolic uncertainty. Out of discussion with Bharti today: (1) a reconstruction based approach targets minimization of a reconstruction error; (2) in hyperbolic space distances between sequence values and their reconstructions vary when varying uncertainty; (3) distance in hyperbolic are exponentially larger if the certainty is larger; (4) a model which feels uncertain about a reconstruction (a model which may be guessing) would prefer to place the reconstruction at a lower uncertainty level; (5) the distance between the gt values and a wrong reconstruction is smaller if the reconstruction is uncertain while exponentially larger if the reconstruction is certain; (6) the model chooses, in a principled way, to mark some  reconstructions as uncertainty, if it feels it could be wrong, because this minimizes the hyperbolic reconstruction error. I hope this is clear. Please give it another iteration with this concept. I'd leave hierarchies out. But ok to name end-to-end.} %Therefore, uncertainty in a hyperspace measures distances in a Poincaré disk and determines where the prediction lies. In other words, the closer the predicted value is to the disk circumference the more certain the model is about the outcome.

By analysing uncertainty in the context of anomaly detection, in this work we provide a novel definition of anomaly detection. A detectable anomaly is an instance where the model is certain about its outcome, but which it reconstructs wrongly. Hence, we intertwine the anomaly status of a particular instance to both its detectability and its corresponding uncertainty in the hyperspace.


The main contributions of this work are:
\begin{itemize} %[noitemsep,topsep=0pt]
\item We propose the first model for anomaly detection based on hyperbolic uncertainty;
%
\item We analyse the model hyperbolic uncertainty in relation to the reconstruction error and discuss the self-regulating principle for self-supervised learning;
%
\item We integrate the estimated uncertainty into a state-of-the-art anomaly detection algorithm, improving the state-of-the-art on established anomaly detection benchmarks and elderly daily routine trajectories.
%
%\item We conduct ablation studies and show that the use of uncertainty as computed from MC dropout is also beneficial. \FG{Take out if not done.}
\end{itemize}

%\BP{Here goes the description of the paper's structure. Will do that in the end}\FG{No need for the paper structure. It's quite a normal paper and of few pages.}






==> sec/Backup/method_bk_2022-02-10.tex <==
\section{Method}
In this section, we first discuss best practises in anomaly detection (Section \ref{sec:background}); then we detail the proposed hyperbolic uncertainty and its use for detecting anomalies (Section \ref{sec:hypAD}); finally we discuss the motivation for it (Section \ref{sec:mot}).


\input{fig/hyperTadGAN.tex}

\subsection{Background}
\label{sec:background}

The current state-of-the-art in univariate anomaly detection is a reconstruction-based technique~\cite{geiger2020tadgan} which additionally leverages a GAN critic score. TadGAN encodes the input data $x$ to a latent space and then decodes the encoded data. This encoding-decoding operation requires two mapping functions $E : X \rightarrow Z$ and $G : Z \rightarrow  X$.
The reconstruction operation can be given as $x \rightarrow E(x) \rightarrow G(E(x)) \rightarrow \widetilde{x} \approx x$. TadGAN leverages adversarial learning to train the two mappings by using two adversarial critics $D_x$ and $D_z$. The goal of $D_x$ is to distinguish between the real and the generated time series, while $D_z$ measures the performance of the mapping into latent space. The model is trained using the combination of Wasserstein loss~\cite{pmlr-v70-arjovsky17a} and Cycle consistency loss~\cite{8237506}. 
%\FG{please better clarity: over the training set?}
%To calculate the anomaly scores, TadGAN first computes the mean and standard deviation of both the scores , and then the normalised scores, $Z_{RE}(x)$ and $Z_D_x(x)$, are computed by subtracting the mean and dividing by standard deviation. 
% \FG{it should be Z?} 
TadGAN computes the reconstruction error $RE(x)$ between x and $\widetilde{x}$ using
three types of reconstruction  functions: \textbf{i.}\ Point-wise difference: considers the difference of values at every time stamp; \textbf{ii.}\ Area difference: is applied on signals of fixed lengths and measures the similarity between local regions; \textbf{iii.}\ Dynamic time warping: additionally handles time gaps between the two signals to calculate the reconstruction error.

To calculate the anomaly score, TadGAN first normalises the reconstruction error and critic scores by subtracting the mean and dividing by standard deviation. The normalised scores, $Z_{RE}(x)$ and $Z_{D_x}(x)$, are then combined using either their convex combination:
\begin{equation}
    s_c(x) = \alpha Z_{RE}(x) + (1 - \alpha) Z_{D_x}(x)
    \label{eq:anomaly_score_sum}
\end{equation}
or their product:
\begin{equation}
    s_p(x) = Z_{RE}(x) \odot Z_{D_x}(x)
    \label{eq:anomaly_score_prod}
\end{equation}

%\BM{An instance is marked as an anomaly if the anomalous score described above is higher than a threshold value. }
%For details, please refer to \cite{geiger2020tadgan}. 

%The anomaly scores are computed by
%using  
%

%\FG{place here a "or" or some connection. I guess it's one or the other, not both.}

%\FG{ Also call then differently $s_c$ and $s_p$ for convex combination and product respectively}
%\FG{Need to clarify that what follows is specific to how the recontruction error is computed, so the Zre, after having reconstructed the signal.}




%\paragraph{Estimating Uncertainty with \textit{Monte Carlo} Dropout}




%\input{fig/hyperTadGAN.tex}


\subsection{Hyperbolic uncertainty for Anomaly detection (HypAD)}
\label{sec:hypAD}

We propose a novel model for anomaly detection in time series based on hyperbolic uncertainty. HypAD is a reconstruction-based model and minimises the reconstruction loss, given by a measure of the hyperbolic distance between the input signal and its reconstruction. In hyperbolic space, errors are exponentially larger when predictions are certain. Therefore, HypAD tends to predict either certain correct reconstructions or uncertain possibly mistaken reconstructions. 

This leads, as we discuss in Sec.~\ref{sec:mot}, to a novel definition of detectable anomaly: i.e. the case of a large reconstruction error with high certainty.



\subsubsection{Hyperbolic Reconstruction Error}
\label{sec:hypRe}

The proposed HypAD is illustrated in Figure~\ref{fig:hypAD}. It integrates the machinery of hyperbolic neural networks into the reconstruction-based architecture of TadGAN. In HypAD the input signal $x$ is first passed through an encoder, then followed by a decoder sub-network. The output of the decoder $G(E(x))$ as well as the original signal $x$ are mapped to the hyperspace, shown as the dotted red edge box with red background. 


An $n$-dimensional hyperspace is a Riemannian geometry with a constant negative sectional curvature. As in~\cite{Khrulkov_2020_CVPR,suris2021hyperfuture}, we adopt the Poincaré ball model of hyperspaces, given by the manifold $\mathbb{D}_n = \{x \in R^n : \|x\| < 1\}$ endowed with the Riemmanian metric $g^\mathbb{D}(x) = \lambda_x^2g^E$,
where $\lambda_x =\frac{2}{1-\|x\|^2}$ is the \textit{conformal factor}
and $g^E = I_n$ is the Euclidean
metric tensor. For details, see~\cite{riemannian,smoothmanifold}.





In order to map $x$ and $G(E(x))$ to the Poincaré ball, we leverage an \textit{exponential map} centered at $\bf{0}$~\cite{suris2021hyperfuture}. This is followed by a hyperbolic feed-forward layer~\cite{NEURIPS2018_dbab2adc} to estimate the corresponding hyperbolic embeddings $h$ and $\widetilde{h}$, shown as solid green boxes in Figure~\ref{fig:hypAD}. Finally, the two hyperbolic embeddings are compared using the Poincaré distance, formulated as follows:
\begin{equation}
{RE}(x)  =  \cosh^{-1}\Bigg(1 + 2{\frac{\|h-\widetilde{h}\|^2}{\big(1-\|h\|^2\big)\big(1-\|\widetilde{h}\|^2\big)}\Bigg)}
\label{eq:poincare}
\end{equation}
%
where $\|h\|^2$ and $\|\widetilde{h}\|^2$ are the distances of the embeddings from the center of the Poincaré ball. %\FG{maybe add: the reconstruction error Z is used both for training and for inference, detecting as anomalies those exceeding a threshold?}
Note that the same reconstruction error function $RE(x)$, is used at training as well as inference time.


\subsubsection{Hyperbolic Uncertainty } 
\label{sec:hypUn}
A key property of the Poincaré ball is that the distance between two points grows exponentially as we move away from the origin. This means that an erroneous reconstruction towards the circumference of the disk is penalised exponentially more than an erroneous reconstruction close to the centre. This leads to the useful tendency of HypAD to either predict a matched reconstruction ($\widetilde{h}$ and $h$ are close by) or an unmatched reconstruction towards the origin ($\widetilde{h}$ and $h$ are far-away, $\|h\|^2$ and $\|\widetilde{h}\|^2$ are small), in order to minimize Eq. \eqref{eq:poincare}.

Hence, the distance of the reconstruction to the origin provides a natural estimate of the model's uncertainty, referred to as hyperbolic uncertainty, $U(X)$, thus formulated:
\begin{equation}
{U}(X)  =  1 - \| \widetilde{h}\|^2
\label{eq:hypUn}
\end{equation}

The smaller the distance from the origin, the more uncertain is the model. 




\subsubsection{Combining Hyperbolic Uncertainty with Reconstruction Error and Critic Score}
\label{sec:combine}

Hyperbolic uncertainty ${U}(x)$ is integrated into the anomaly score as follows:
\begin{equation}
    s_u(x) =  Z_{RE}(x) \odot Z_{D_x}(x) \odot (1-{U}(x))
    \label{eq:uncer}
\end{equation}

Equation \ref{eq:uncer} brings together the reconstruction error $Z_{RE}(x)$ (the larger the error, the more likely the anomaly) with the critic score $Z_{D_x}(x)$ (larger critic scores point to anomalies) and the model certainty: $1-{U}(x)$.

The simple multiplication formulation of the certainty of the model reduces the scores of anomalies when HypAD is not confident of the reconstructions. While being simple, this outperforms the current state-of-the-art, as we show in Section~\ref{sec:expres}.


\subsection{Motivation for HypAD}
\label{sec:mot}

HypAD takes motivation from a key idea: \textit{a detectable anomaly is one where the model is certain, and which it predicts wrongly}. In other words, if the model encounters a known pattern, which it knows how to reconstruct, then it will call it anomalous, if the reconstruction does not match the input signal.

The principled formulation of hyperbolic uncertainty is paramount towards this goal: HypAD predicts a reconstruction as uncertain if it is doubtful that it may be wrong.

\input{fig/cosine_barplot.tex}

\BM{Figure~\ref{fig:cosine_barplot} illustrates this key concept for all the datasets. The first, second and third rows correspond to the univariate, U-CASAS and SWaT datasets respectively.}
The bar plot depicts the average cosine distances between the input signals and their reconstructions, against specific intervals of certainty, along the x-axis.
The higher the cosine distances, the more distinct the reconstruction is from the provided signals\footnote{The Poincaré ball model is conformal to the Euclidean space and it preserves the same angles~\cite{shimizu2021hyperbolic}.}. 
\BM{
Note that for the first two rows, the initial three plots (columns) correspond to the signals that report the best improvement in F1-score and the last plot corresponds to the signal with worst improvement. Since SWaT contains only a single long-term signal, we report only its
corresponding bar-plot.} 


Observe \BM{in the second row}, how HypAD learns to correctly assign lower certainty to wronger estimates for the cases of Fall, Weakness, and Nocturia. For the last signal SlowerWalking, HypAD fails to learn a meaningful uncertainty and labels all reconstructions as certain. It is however notable that the representation is still interpretable and the case of failure discernible. 

\BM{Similar trends can be seen for the case of Univariate and SWaT datasets.} 

%One from these two is also a case where HypAD underperforms. 




%Figure~\ref{fig:cosine_barplot} illustrates this key concept for all the multi-variate sequences of the U-CASAS dataset (see details in Sec. \ref{sec:dataset}).

%The bar plot depicts the average cosine distances between the input signals and their reconstructions, against specific intervals of certainty, along the x-axis. The higher the cosine distances, the more distinct the reconstruction is from the provided signals\footnote{The Poincaré ball model is conformal to the Euclidean space and it preserves the same angles~\cite{shimizu2021hyperbolic}.}. Observe how HypAD learns to correctly assign lower certainty to wronger estimates for the cases of Fall, Weakness, and Nocturia. For two of the multivariate datasets, HypAD fails to learn a meaningful uncertainty and labels all reconstructions as certain. One from these two is also a case where HypAD underperforms. It is however notable that the representation is still interpretable and the case of failure discernible.





%

\input{tab/datasets}






==> tab/ablation_multivariate.tex <==
\begin{table}[t]
\centering
\caption{The average F1 score and g-measure across the multivariate datasets (U-CASAS), using different combinations for anomaly detection. $Z_{RE}$, $ Z_{D_x}$  and  $(1-U)$ represent the normalised reconstruction error, critic score and certainty of the model, respectively. The bold-faced entry depicts the proposed strategy in this paper.}
\label{tab:ablation_multivariate}
\resizebox{.47\textwidth}{!}{%
\begin{tabular}{llcc}
\multicolumn{2}{l}{} & F1 ($\mu\pm\sigma$) & g-measure ($\mu\pm\sigma$)\\ \hline
\multicolumn{2}{l}{ $ Z_{D_x} $} & 0.050 $\pm$ 0.128 & 0.058 $\pm$ 0.111 \\

\multicolumn{2}{l}{ $ Z_{D_x} \odot (1-U) $} &  0.117 $\pm$ 0.162 &  0.129 $\pm$ 0.177 \\ 

\multicolumn{2}{l}{ $Z_{RE}$} & 0.409 $\pm$ 0.163 & 0.466 $\pm$ 0.126\\
\multicolumn{2}{l}{ $Z_{RE} \odot (1-U) $} & 0.423 $\pm$ 0.166 & 0.516 $\pm$ 0.191 \\

\multicolumn{2}{l}{ $Z_{RE} \odot Z_{D_x} $} & 0.397 $\pm$ 0.094 & 0.497 $\pm$ 0.074\\

\multicolumn{2}{l}{ $Z_{RE} \odot Z_{D_x} \odot (1-U) $} &  \textbf{0.428 $\pm$ 0.123} &  \textbf{0.520 $\pm$ 0.095} \\ 

%\multicolumn{2}{l}{{AE (rec\_error$\times$certainty)}} & 0.067 $\pm$ 0.059 &  0.073 $\pm$ 0.06\\ 
%\multicolumn{2}{l}{{LstmAE (rec\_error$\times$certainty)}} & 0.068 $\pm$ 0.045 &  0.151 $\pm$ 0.054\\ 
%\multicolumn{2}{l}{{ConvAE (rec\_error$\times$certainty)}} & 0.097 $\pm$ 0.077 &  0.18 $\pm$ 0.102\\ 

% \bottomrule
% \hline
% \multicolumn{2}{l}{} & \begin{tabular}[c]{@{}c@{}}g-measure ($\mu\pm\sigma$)\end{tabular} &\\ 
% \hline
% \multicolumn{2}{l}{HypAD (rec\_error)} & 0.466 $\pm$ 0.126 &\\
% \multicolumn{2}{l}{HypAD (rec\_error$\times$critic\_score)} & 0.497 $\pm$ 0.074 &\\
% \multicolumn{2}{l}{HypAD (rec\_error$\times$certainty)} & 0.516 $\pm$ 0.191 &\\
% \multicolumn{2}{l}{\textbf{HypAD (rec\_error$\times$critic\_score$\times$certainty)}} & 0.520 $\pm$ 0.095 &\\ 
\hline
%\bottomrule
\end{tabular}%
}
\end{table}

==> tab/ablation_univariate.tex <==
\begin{table}[t]
\centering
\caption{The average F1 score across different univariate datasets, using different combinations for anomaly detection. $Z_{RE}$, $ Z_{D_x}$  and  $(1-U)$ represent the normalised reconstruction error, critic score and certainty of the model, respectively. The bold-faced entry depicts the proposed strategy in this paper.}
\label{tab:ablation_univariate}
\resizebox{.32\textwidth}{!}{%
\begin{tabular}{llc}
\multicolumn{2}{l}{} & F1 ($\mu\pm\sigma$) \\ \hline
\multicolumn{2}{l}{ $Z_{D_x}$} & 0.169 $\pm$ 0.220 \\ 
\multicolumn{2}{l}{ $Z_{D_X} \odot (1-U) $}  & 0.189 $\pm$ 0.230 \\

\multicolumn{2}{l}{ $Z_{RE}$} & 0.574 $\pm$ 0.099 \\ 
\multicolumn{2}{l}{ $Z_{RE} \odot (1-U) $}  & 0.592 $\pm$ 0.086 \\

\multicolumn{2}{l}{  $Z_{RE} \odot Z_{D_x} $} & 0.604 $\pm$ 0.062 \\

\multicolumn{2}{l}{$Z_{RE} \odot Z_{D_x} \odot (1-U) $} & \textbf{0.631 $\pm$ 0.075} \\ \hline
\end{tabular}%
}
\end{table}




% \begin{table}[]
% \centering
% \caption{Ablation study of HypAD on the multivariate datasets (U-CASAS). The bold-faced entry depicts the proposed strategy in this paper.}
% \label{tab:ablation_multivariate}
% \resizebox{.47\textwidth}{!}{%
% \begin{tabular}{llc}
% \multicolumn{2}{l}{} & F1 ($\mu\pm\sigma$) \\ \hline
% \multicolumn{2}{l}{HypAD (rec\_error)} &  \\
% \multicolumn{2}{l}{HypAD (rec\_error$\times$critic\_score)} & 0.397 $\pm$ 0.094 \\
% \multicolumn{2}{l}{HypAD (rec\_error$\times$certainty)} &  \\
% \multicolumn{2}{l}{\textbf{HypAD (rec\_error$\times$critic\_score$\times$certainty)}} & 0.461 $\pm$ 0.117 \\ \hline
% \end{tabular}%
% }
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
%\begin{table}[]
%\centering
%\caption{Ablation study of HypAD on the multivariate datasets (U-CASAS). The bold-faced entry depicts the proposed strategy in this paper.}
%\label{tab:ablation_multivariate}
%\resizebox{.47\textwidth}{!}{%
%\begin{tabular}{llcc}
%\multicolumn{2}{l}{} &
%  \begin{tabular}[c]{@{}c@{}}F1\\ ($\mu\pm\sigma$)\end{tabular} &
%  \begin{tabular}[c]{@{}c@{}}g-measure\\ ($\mu\pm\sigma$)\end{tabular} \\ \hline
%\multicolumn{2}{l}{HypAD (rec\_error)}                      & 0.409 $\pm$ 0.163 & 0.466 $\pm$ 0.126 \\
%\multicolumn{2}{l}{HypAD (rec\_error$\times$critic\_score)} & 0.397 $\pm$ 0.094 & 0.497 $\pm$ 0.074 \\
%\multicolumn{2}{l}{HypAD (rec\_error$\times$certainty)}     & 0.423 $\pm$ 0.166 & 0.516 $\pm$ 0.191 \\
%\multicolumn{2}{l}{HypAD (rec\_error$\times$critic\_score$\times$certainty)} &
%  0.461 $\pm$ 0.117 &
%  0.511 $\pm$ 0.090 \\ \hline
%\end{tabular}%
%}
%\end{table}



% Please add the following required packages to your document preamble:
% \usepackage{graphicx}


==> tab/datasets_bak.tex <==
\begin{table*}[h]
\centering
\caption{Dataset summary \AF{add SWAT and make words shorter}}
\label{tab:datasets}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llcccccccccccccccc}
\multicolumn{2}{l}{\multirow{3}{*}{}} & \multicolumn{11}{c}{Univariate} & \multicolumn{5}{c}{Multivariate} \\ \cline{3-18} 
\multicolumn{2}{l}{} & \multicolumn{2}{c}{NASA} & \multicolumn{4}{c}{Yahoo} & \multicolumn{5}{c}{NAB} & \multicolumn{5}{c}{CASAS} \\ \cline{3-18} 
\multicolumn{2}{l}{} & SMAP & \multicolumn{1}{c}{MSL} & A1 & A2 & A3 & \multicolumn{1}{c}{A4} & Art & AdEx & AWS & Traf & \multicolumn{1}{c}{Tweets} & Fall & MoreTimeInChair & Weakness & SlowerWalking & Nocturia \\ \hline
\multicolumn{2}{l}{Num. of signals} & 53 & \multicolumn{1}{c}{27} & 67 & 100 & 100 & \multicolumn{1}{c}{100} & 6 & 5 & 17 & 7 & \multicolumn{1}{c}{10} & 1 & 1 & 1 & 1 & 1 \\
\multicolumn{2}{l}{Num. of anomalies} & 67 & \multicolumn{1}{c}{36} & 178 & 200 & 939 & \multicolumn{1}{c}{835} & 6 & 11 & 30 & 14 & \multicolumn{1}{c}{33} & 2 & 2 & 4 & 2 & 2 \\
 & Point anomalies & 0 & \multicolumn{1}{c}{0} & 68 & 33 & 935 & \multicolumn{1}{c}{833} & 0 & 0 & 0 & 0 & \multicolumn{1}{c}{0} & 0 & 0 & 0 & 0 & 0 \\
 & Collective anomalies & 67 & \multicolumn{1}{c}{36} & 110 & 167 & 4 & \multicolumn{1}{c}{2} & 6 & 11 & 30 & 14 & \multicolumn{1}{c}{33} & 2 & 2 & 4 & 2 & 2 \\
\multicolumn{2}{l}{Num. of anomaly points} & 54,696 & \multicolumn{1}{c}{7,766} & 1,699 & 466 & 943 & \multicolumn{1}{c}{837} & 2,418 & 795 & 6,312 & 1,560 & \multicolumn{1}{c}{15,651} & 99 & 239 & 1,248 & 276 & 1,060 \\
 & Num. out of distribution & 18,126 & \multicolumn{1}{c}{642} & 861 & 153 & 21 & \multicolumn{1}{c}{49} & 123 & 15 & 210 & 86 & \multicolumn{1}{c}{520} & - & - & - & - & - \\
 & Percentage of total & 33.1\% & \multicolumn{1}{c}{8.3\%} & 51.6\% & 32.8\% & 2.2\% & \multicolumn{1}{c}{5.9\%} & 5.1\% & 1.9\% & 3.3\% & 5.5\% & \multicolumn{1}{c}{3.3\%} & - & - & - & - & - \\
\multicolumn{2}{l}{Num. of instances} & $\sim563$k & \multicolumn{1}{c}{$\sim132$k} & $\sim95$k & $\sim142$k & 168k & \multicolumn{1}{c}{168k} & $\sim24$k & $\sim8$k & $\sim68$k & $\sim16$k & \multicolumn{1}{c}{$\sim159$k} & $\sim54$k & $\sim276$k & $\sim39$k & $\sim39$k & $\sim39$k \\
\multicolumn{2}{l}{Synthetic?} & No & \multicolumn{1}{c}{No} & No & Yes & Yes & \multicolumn{1}{c}{Yes} & Yes & No & No & No & \multicolumn{1}{c}{No} & No & No & No & No & No \\ \hline
\end{tabular}%
}
\end{table*}
